Symmetric Rank-One Quasi-Newton Methods for Deep Learning Using Cubic Regularization

Stochastic gradient descent and other first-order variants, such as Adam and AdaGrad, are commonly used in the field of deep learning due to their computational efficiency and low-storage memory requirements. However, these methods do not exploit curvature information. Consequently, iterates can converge to saddle points or poor local minima. On the other hand, Quasi-Newton methods compute Hessian approximations which exploit this information with a comparable computational budget. Quasi-Newton methods re-use previously computed iterates and gradients to compute a low-rank structured update. The most widely used quasi-Newton update is the L-BFGS, which guarantees a positive semi-definite Hessian approximation, making it suitable in a line search setting. However, the loss functions in DNNs are non-convex, where the Hessian is potentially non-positive definite. In this paper, we propose using a limited-memory symmetric rank-one quasi-Newton approach which allows for indefinite Hessian approximations, enabling directions of negative curvature to be exploited. Furthermore, we use a modified adaptive regularized cubics approach, which generates a sequence of cubic subproblems that have closed-form solutions with suitable regularization choices. We investigate the performance of our proposed method on autoencoders and feed-forward neural network models and compare our approach to state-of-the-art first-order adaptive stochastic methods as well as other quasi-Newton methods.x

==> Sections/Experimentation.tex <==
The following algorithm is used to run experiments on different datasets given in Section \ref{sec:Experiments}.

\begin{algorithm}
	\caption{Forward and backward pass of DNN for a single data-point}
	\begin{algorithmic}
		\State \textbf{Given} input ($x$,$y$), weights (and biases) $\Theta_{l}$ and activations $\sigma_l$ where $l \in [1,L]$ is the layer and $L$ is the number of layers
		\State  $\mathbf{a}_0 = x$; 
		\For {$l=1, \ldots, L$}{ $h_l = \Theta_l a_{l-1};$}{$a_l = \sigma_{l}(h_l)$}
		\EndFor
		\State {$\dot{a}_L \overset{\text{def}}{=}\nabla_z a_L \leftarrow \frac{\partial \mathcal{L}(z,y)}{\partial z}\rvert_{z=a_L}$}
		\For {$l=1, \ldots, L$} {$g_l = \dot{a}_l \bigodot \sigma'(h_l)$};{$ \dot{\Theta}_l = g_i \hat{a}^{\top}_{i-1};$}{$\dot{a}_{l-1} = \Theta_l^\top g_l$}
		\EndFor
	\end{algorithmic}\label{alg:DNN}
\end{algorithm}
We present the learning rates for the different algorithms used in Table (\ref{tbl:lr}):
\begin{table}[h]
	\centering
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\textbf{Method} & 
		Adam &  
		SGD & 
		Adagrad &
		RMSProp & 
		L-BFGS \\
		\hline
		\textbf{Learning rate} & 
		$1.0 \times 10^{-3}$ &
		$1.0 \times 10^{-1}$  & 
		$1.0 \times 10^{-2}$ & 
		$1.0 \times 10^{-2}$ & 
		$1.0 \times 10^0$ \\
		\hline
	\end{tabular}
	\caption{Learning rates for each update rule.}
	\label{tbl:lr}
\end{table}

For the MNIST dataset, the architecture is presented in detail in Table \ref{tbl:mnistnetwork}.
For Fashion-MNIST (FMNIST), the network is described in Table \ref{tbl:fmnist-network}.
For CIFAR10, the network architecture is described in Table \ref{tbl:CIFAR10-networks}.
For the autoencoder, we use the architecture presented in Table \ref{tbl:AutoEncMNIST}.
Finally, the same network architecture is used for reconstruction of FMNIST images.


\begin{table*}[!h]
	\centering
	\resizebox{0.6\textwidth}{!}{
		\begin{tabular}{c}
			\begin{tabular}{|c|c|c|c|c|c|}
				\hline
				\multicolumn{6}{|c|}{\small{MNIST network }}\\
				\hline\hline
				Layer& In & Out&Kernel& Stride&Padding\\
				\hline
				Linear & 784 & 500 & - & - & -\\
				ReLU & 500 & 500 & - & - & -\\
				Dropout & - & - & - & - &-\\
				Linear & 500 & 10 & - & - & -\\
				SoftMax & 10 & 10 & - & - & - \\
				\hline
			\end{tabular}\\
			\\[-.15cm]
	\end{tabular}}\caption{Network architecture for MNIST.}\label{tbl:mnistnetwork}
\end{table*}

\begin{table*}[!h]
	\centering
	\resizebox{0.6\textwidth}{!}{
		\begin{tabular}{c}
			\begin{tabular}{|c|c|c|c|c|c|}
				\hline
				\multicolumn{6}{|c|}{\small{F-MNIST network }}\\
				\hline\hline
				Layer& In & Out&Kernel& Stride&Padding\\
				\hline
				Conv2d & 1 & 10 & 5 $\times$ 5 & 1 & None\\
				MaxPool2d & - & - & 2 $\times$ 2 & - & -\\
				ReLU & - & - & - & - & -\\
				Conv2d & 10 & 20 & 5 $\times$ 5 & 1 & None\\
				MaxPool2d & 10 & 10 & 2 $\times$ 2 & - & -\\
				ReLU & - & - & - & - & -\\
				Dropout & - & - & - & - &-\\
				Linear & 320 & 50 & - & - & -\\
				Linear & 50 & 10 & - & - & - \\
				LogSoftmax & 50 & 10 & - & - & - \\
				\hline
			\end{tabular}\\
			\\[-.15cm]
	\end{tabular}}\caption{Network architecture for FMNIST.}\label{tbl:fmnist-network}
\end{table*}


\begin{table*}[!h]
	\centering
	\resizebox{0.6\textwidth}{!}{
		\begin{tabular}{c}
			\begin{tabular}{|c|c|c|c|c|c|}
				\hline
				\multicolumn{6}{|c|}{\small{CIFAR10 network}}\\
				\hline\hline
				Layer& In & Out&Kernel& Stride&Padding\\
				\hline
				Conv2d & 3 & 6 & 5 $\times$ 5 & 1 & None\\
				MaxPool2d & - & - & 2 $\times$ 2 & - & -\\
				ReLU & - & - & - & - & -\\
				Conv2d & 6 & 16 & 5 $\times$ 5 & 1 & None\\
				MaxPool2d & 10 & 10 & 2 $\times$ 2 & - & -\\
				ReLU & - & - & - & - & -\\
				Linear & 120 & 84 & - & - & -\\
				Linear & 84 & 10 & - & - & - \\
				LogSoftmax & 50 & 10 & - & - & - \\
				\hline
			\end{tabular}\\
			\\[-.15cm]
	\end{tabular}}\caption{Network architecture for CIFAR10.}\label{tbl:CIFAR10-networks}
\end{table*}

\begin{table*}[!h]
	\centering
	\resizebox{0.6\textwidth}{!}{
		\begin{tabular}{c}
			\begin{tabular}{|c|c|c|c|c|c|}
				\hline
				\multicolumn{6}{|c|}{\small{MNIST-Autoencoder}}\\
				\hline\hline
				Layer& In & Out&Kernel& Stride&Padding\\
				\hline
				Conv2d & 1 & 8 & 3 $\times$ 3 & 2 & 1\\
				ReLU & - & - & - & - & -\\
				Conv2d & 8 & 16 & 3 $\times$ 3 & 2 & 1\\
				BatchNorm & - & - & - & - & -\\
				ReLU & - & - & - & - & -\\
				Conv2d & 16 & 32 & 3 $\times$ 3 & 2 & 0\\
				Linear & 288 & 128 & - & - & -\\
				ReLU & - & - & - & - & -\\
				Linear & 128 & 4 & - & - & - \\
				Linear & 4 & 128 & - & - & - \\
				ReLU & - & - & - & - & -\\
				Linear & 128 & 288 & - & - & - \\
				ReLU & - & - & - & - & -\\
				ConvTrans2d & 32 & 16 & 3 $\times$ 3 & 2 & 0\\
				BatchNorm & - & - & - & - & -\\
				ReLU & - & - & - & - & -\\
				ConvTrans2d & 16 & 8 & 3 $\times$ 3 & 2 & 1\\
				BatchNorm & - & - & - & - & -\\
				ReLU & - & - & - & - & -\\
				ConvTrans2d & 8 & 1 & 3 $\times$ 3 & 2 & 1\\
				
				
				\hline
			\end{tabular}\\
			\\[-.15cm]
	\end{tabular}}\caption{Network architecture for Fashion-MNIST Autoencoder operation.}\label{tbl:AutoEncMNIST}
\end{table*}


\newpage

\null

\vfill

\newpage



==> Sections/LSR1Broyden.tex <==
\begin{equation*}
	B_{k+1}s_k = y_k,
\end{equation*}
To better understand the SR1 update, we write down the Broyden class of updates  as follows:
\begin{equation}\label{eqn:SR1}
	B_{k+1} = B_k - \frac{1}{s_k^TB_ks_k}B_ks_ks_k^TB_k + \frac{1}{y_k^Ts_k}y_ky_k^T + \phi(s_k^TB_k s_k)v_kv_k^T,
\end{equation}
where
\begin{equation*}
	v_k = \frac{y_k}{y_k^Ts_k} - \frac{B_ks_k}{s_k^TB_ks_k}.
\end{equation*}
The SR1 update from \eqref{eqn:SR1} is obtained by setting $\phi = y_k^Ty_k/(y_k^T - s_k^TB_ks_k)$; in this case,

\begin{equation*}
	B_{k+1} = B_k + \frac{1}{s_k^T(y_k - B_ks_k)}(y_k -B_ks_k)(y-B_ks_k)^T
\end{equation*}

==> Sections/ProposedApproach.tex <==
We begin by discussing the SR1 update and the adaptive regularizion using cubics methods for large-scale optimization.

\noindent\textbf{The SR1 update.} The SR1 update is a unique rank-one update in Broyden class satisfying the \textit{secant equation}. The interesting part about the SR1 matrices is that it produces a sequence of possibly indefinite matrices which makes it appealing to deep learning applications where $\mathbf{f}$ is non-convex.

==> Sections/Solution.tex <==
%We define the optimization problem as follows:
%\begin{equation}
%	\underset{x \in \mathbb{R}^n}{\text{min}} f(\Theta)
%\end{equation}
%
%This can be decomposed to the following:
%\begin{equation*}
%\underset{\bar{\mathbf{s}}\in \mathbb{R}^n}{\text{min}} \bar{\mathbf{m}}(\bar{\mathbf{s}}) = \sum\limits_{i=1}^{n} \underset{\bar{\mathbf{s}}_i}{\text{min}} \left( \bar{\mathbf{g}}_i\bar{\mathbf{s}}_i  + \frac{\lambda_i}{2} \bar{\mathbf{s}}_i^2 + \frac{\mu}{3} |\bar{\mathbf{s}_i}|^3\right)
%\end{equation*}
%
%We re-write the solution from Algorithm \ref{alg:LSR1ARC} as $\bar{\mathbf{s}}^{*} = - \mathbf{C}\bar{\mathbf{g}}$, where $\mathbf{C} = diag(c_1, \ldots, c_n)$ and $c_i = \frac{2}{\lambda_i + \sqrt{\lambda_i^2 + 4\mu|\bar{\mathbf{g}}_{i}|}}$. We provide the complete formulation and solution to the subproblem in sections \ref{sec:B0}, \ref{sec:limsetting} and \ref{sec:closedformsolve}
%
%\subsection{Limited-memory}\label{sec:limsetting}
%We acknowledge that a $n \times n$ Hessian approximation cannot be stored. Hence we propose a limited-memory solution. We use the compact representation equation (\ref{eqn:compactSR1}) to define our approximation update. Now, $\Psi$ is an $m \times n$ matrix where $m \ll n$. We perform a `thin' QR-decomposition on $\Psi = \mathbf{Q}\mathbf{R}$. This yields
%
%
%\begin{equation*}	
%\mathbf{B}_{k+1} \ = \ \mathbf{B}_0 + 
%	\begin{bmatrix}
%	\\
%	\mathbf{Q}_{k+1}\mathbf{R}_{k+1}  \\
%	\phantom{t}
%	\end{bmatrix}
%	\hspace{-.3cm}
%	\begin{array}{c}
%	\left  [ \  \mathbf{M}_{k+1}^{\phantom{h}}  \right ] \\
%	\\
%	\\
%	\end{array}
%	\hspace{-.3cm}
%	\begin{array}{c}
%	\left [  \ \quad \mathbf{R}_{k+1}^{\top}\mathbf{Q}_{k+1}^{\top}\quad \ \right ] \\
%	\\
%	\\
%	\end{array},
%\end{equation*}
%where $\mathbf{R} \in \mathbb{R}^{m \times m}$, $\mathbf{Q} \in \mathbb{R}^{m \times n}$. Next, we compute the spectral decomposition on the matrix $\mathbf{RMR}^\top$ to yield $\mathbf{P}\Lambda \mathbf{P}^\top$. We define $\mathbf{U}_\parallel = \mathbf{QP}$ and form the following representation:
%\begin{equation*}
%\mathbf{B}_{k+1} \ = \ \mathbf{B}_0 + 
%	\begin{bmatrix}
%	\\
%	\mathbf{U_{\parallel}} \\
%	\phantom{t}
%	\end{bmatrix}
%	\hspace{-.3cm}
%	\begin{array}{c}
%	\left  [ \  \Lambda^{\phantom{h}}  \right ] \\
%	\\
%	\\
%	\end{array}
%	\hspace{-.3cm}
%	\begin{array}{c}
%	\left [  \ \quad \mathbf{U}_{\parallel}^{\top}\quad \ \right ] \\
%	\\
%	\\
%	\end{array}.
%\end{equation*}
%
%\subsection{Dynamic initialization of $\mathbf{B}_0$}\label{sec:B0} 
%
%We define $\mathbf{B}_0 = \delta \mathbf{I}$, where $\delta = 0 < \delta < \hat{\lambda}_i $.
%$\hat{\lambda}_i$ denotes the smallest eigenvalue of the generalized eigenvalue problem 
%\begin{equation*}
%	(\mathbf{D}_k + \mathbf{L}_k + \mathbf{L}_k^{\top})\mathbf{u} = \hat{\lambda}_i \mathbf{S}^{\top}_k \mathbf{S}_k \mathbf{u}
%\end{equation*}
%For further information, refer to \cite{Erway2020TrustregionAF} (Lemma 2.4)
%
%\subsection{Closed-form solution}\label{sec:closedformsolve}
%Now we are ready to discuss the closed-form solution of the cubic-regularized model. Suppose we approximate a $n \times n$ Hessian. The closed form solution in the new space of variables is given by
%\begin{equation*}
%	\bar{\mathbf{s}}^* = -\mathbf{\mathbf{C}}\bar{\mathbf{g}}.
%\end{equation*}
%Here, $\mathbf{C} = diag(c_1,\ldots, c_n)$ and $c_i \overset{\text{def}}{=} \frac{2}{\lambda_i^2 + \sqrt{\lambda_i^2 + 4 \mu |\bar{g}_i|}}$, where $\bar{\mathbf{g}} = \mathbf{U}^\top \mathbf{g}$. To get the closed form solution in the original space, we transform the new space back to the original space as
%\begin{equation*}
%	\mathbf{s}^* = \mathbf{U} \bar{\mathbf{s}}^*.
%\end{equation*}
%However, we only operate on a limited memory approximation of the Hessian. We define $\mathbf{U} = [ \mathbf{U}_\parallel, \mathbf{U}_\perp] \in \mathbb{R}^{n \times n}$, where we only operate on $\mathbf{U}_\parallel$. Thus the formulation is defined as 
%\begin{align*}
%	\mathbf{B}u &= \delta \mathbf{u},\\
%	\mathbf{B}u &= (\delta +\lambda_i) \mathbf{u},
%\end{align*}
%where $\delta$ is computed using the formulation described in \ref{sec:B0} and $\lambda_i$ is defined by the eigen value decomposition in . Thus the solution in the new space is given by,
%\begin{align*}
%	\bar{\mathbf{s}}_\parallel^{*} = \mathbf{U}_{\parallel}^{\top}\mathbf{s}^{*},\quad \bar{\mathbf{s}}^{*}_{\perp} = \mathbf{U}_{\perp}^{\top}\mathbf{s}^{*},\\
%	\bar{\mathbf{g}}_{\parallel} = \mathbf{U}_{\parallel}^{\top}\mathbf{g}, \quad \bar{\mathbf{g}}_{\perp} = \mathbf{U}_{\perp}^{\top}\mathbf{g}.
%\end{align*}
%We make the following observations:
%\begin{enumerate}
%	\item $\delta$ is a multiple eigen value. This means $\mathbf{U}_{\perp}$ is not uniquely defined.
%	\item $\mathbf{s}^*$ depends on the choice of $\mathbf{U}_{\perp}$.
%	\item $\bar{\mathbf{g}}_{\perp}$ is used for computing $\bar{\mathbf{s^{*}}}_{\perp}$ and it requires $\mathbf{U}_{\perp}^{\top}\mathbf{g}$.
%\end{enumerate} 
%
%$\mathbf{U}_{\perp}^{\top}\mathbf{g}$ may be prohibitively expensive to compute and store, unless $\mathbf{U}_{\perp}$ is chosen in a special way. We define $\mathbf{g}_{\perp} = (\mathbf{I}_n - \mathbf{U}_{\parallel} \mathbf{U}_{\parallel}^{\top})\mathbf{g}$ which can be re-written as $\mathbf{g}_{\perp} =\mathbf{g} - \mathbf{U}_{\parallel} \mathbf{g}_{\parallel}$.
%
%\subsection{Adaptive regularized cubics}
Once we compute the step in Algorithm \ref{alg:LSR1ARC}, we compute the ratio between the reduction in the actual objective function and the reduction in the model  defined by
		\begin{equation}\label{eq:ratio}
		\rho_k = (f(\Theta_k) - f(\Theta_{k+1}))/(m(\mathbf{s}^*)).
		\end{equation}
where
\begin{equation*}
m(\mathbf{s}^*) = q(\mathbf{s}^*) + \frac{\mu}{3} (\norm{\mathbf{C}_\parallel \bar{\mathbf{g}}_{\parallel}}_3^3 + (\alpha^*)^3\norm{\mathbf{g}_{\perp}}_2^3).
\end{equation*}
and
$$q(\mathbf{s}^*) = \bar{\mathbf{g}}_\parallel^{\top}(\mathbf{C}_{\parallel}^2 \Lambda_{\parallel} + \mathbf{C}_{\parallel}\bar{\mathbf{g}}_{\parallel} + \frac{\delta_k(\alpha^{\star})^2 - 2\alpha^*}{2} \norm{\mathbf{g}_{\perp}}.
$$



==> Sections/cubic.tex <==



Here, we demonstrate how the cubic subproblem
\begin{equation}\label{eqn:modcr0}\tag{8}
	\underset{\bar{\mathbf{s}} \in \mathbb{R}^n}{\text{min}} \  \ \bar{{m}}_{k} (\bar{\mathbf{s}})
	= \bar{\mathbf{g}}_k^\top\bar{\mathbf{s}}
	+ \frac{1}{2}\bar{\mathbf{s}}^\top \mathbf{\Lambda}_k\bar{\mathbf{s}}
	+ \frac{\mu_k}{3}\norm{\bar{\mathbf{s}}}_3^3
\end{equation}
is solved analytically.  Note that $\bar{m}_k(\bar{\mathbf{s}})$ is a separable function,  
meaning we can write $\bar{m}_k(\bar{\mathbf{s}})$ as
$$
	\bar{m}_k(\bar{\mathbf{s}})
	=
	\sum_{i=1}^n
	\left \{
	(\bar{\mathbf{g}}_k)_i (\bar{\mathbf{s}})_i
	+
	\frac{1}{2}(\mathbf{\Lambda}_k)_i(\bar{\mathbf{s}})_i^2
	+
	\frac{\mu_k}{3} |(\bar{\mathbf{s}})_i |_3^3
	\right \}.
$$
Consequently, we can  solve (\ref{eqn:modcr}) by solving one-dimensional problems 
of the form 
\begin{equation}\label{eqn:modcr1}
	\underset{s \in \mathbb{R}}{\text{min}}  \ \ m(s)
	= gs  
	+ \frac{1}{2}\lambda s^2
	+ \frac{\mu_k}{3}|s|^3,
\end{equation}
where $g \in \mathbb{R}$ corresponds to entries in $\bar{\mathbf{g}}_k$ and
$\lambda \in \mathbb{R}$ corresponds to diagonal entries in $\mathbf{\Lambda}_k$.  

To find the minimizer of (\ref{eqn:modcr1}), we first write $m(s)$ as follows:
\begin{equation*}
	m(s) = 
	\begin{cases}
		m_+(s) = gs  
	+ \frac{1}{2}\lambda s^2
	+ \frac{\mu_k}{3}s^3 & \text{if $s \ge 0$}, \\
		m_-(s) = gs  
	+ \frac{1}{2}\lambda s^2
	- \frac{\mu_k}{3}s^3 & \text{if $s \le 0$}. 	
	\end{cases}
\end{equation*}
The corresponding derivative is given by
\begin{equation*}
	m'(s) = 
	\begin{cases}
		m_+'(s) = g
	+ \lambda s
	+ \mu_ks^2 & \text{if $s \ge 0$},\\
		m_-'(s) = g 
	+ \lambda s
	- \mu_ks^2 & \text{if $s \le 0$}.
	\end{cases}
\end{equation*}
The minimizer $s^*$ of $m(s)$ is obtained by setting $m'(s)$ to zero and will depend on the sign of $g$ because $g$ is the slope of $m(s)$ at $s = 0$, i.e., $m'(0) = g$.  
In particular,
if $g > 0$, then $s^*$  is the minimizer of $m_-(s)$ (see Figs.\ \ref{fig:cubic}(a) and (c)), namely
\begin{equation*}
	s^* = \frac{-\lambda + \sqrt{\lambda^2 + 4gu}}{-2\mu}.
\end{equation*}
If $g < 0$, then $s^*$ is the minimizer of $m_+(s)$ (see Figs.\ \ref{fig:cubic}(b) and (d)), which is given by
\begin{equation*}
	s^* = \frac{-\lambda + \sqrt{\lambda^2 - 4gu}}{2\mu}.
\end{equation*}
Note that these two expressions
for $s^*$ are equivalent to the following formula:
$$
	s^* = \frac{-2g}{\lambda + \sqrt{\lambda^2 + 4|g|\mu}}.
$$






\begin{figure}[ht!]
	\begin{tabular}{cc}
	\includegraphics[width=3.75cm, trim={2cm 1cm 2cm 0},clip]{Figures/cubic1.pdf} &
	\includegraphics[width=3.75cm, trim={2cm 1cm 2cm 0},clip]{Figures/cubic2.pdf}  \\
	(a) $\lambda > 0$ and $g > 0$ & (b) $\lambda > 0$ and $g < 0$ \\
	\includegraphics[width=3.75cm, trim={2cm 1cm 2cm 0},clip]{Figures/cubic3.pdf} &
	\includegraphics[width=3.75cm, trim={2cm 1cm 2cm 0},clip]{Figures/cubic4.pdf} \\
	(c) $\lambda < 0$ and $g > 0$ & (d)  $\lambda < 0$ and $g < 0$
	\end{tabular}
	\caption{Illustration of the piece-wise cubic function $m(s)$. When $\lambda > 0$, 
	$m(s)$ is a convex function and has a unique local minimum, which is also the global minimum 
	((a) and (b)).
	If $\lambda < 0$, then $m(s)$ has two local minima ((c) and (d)).
	The scalar $g$ corresponds to the slope of $m(s)$ at $s = 0$, i.e., $m'(0) = g$.
	If $g > 0$, the minimum $s^*$ of $m(s)$
	corresponds to the minimum of $m_-(s)$ (black circle in (a) and (c)), 	
	and if $g < 0$, then $s^*$ corresponds to the minimum of $m_+(s)$ (red circle in (b) and (d)).
	\label{fig:cubic}}
\end{figure}








